Towards a Semantics-Aware Code Transformation Toolchain for Heterogeneous Systems

Obtaining good performance when programming heterogeneous computing platforms poses significant challenges. We present a program transformation environment, implemented in Haskell, where architecture-agnostic scientific C code with semantic annotations is transformed into functionally equivalent code better suited for a given platform. The transformation steps are represented as rules that can be fired when certain syntactic and semantic conditions are fulfilled. These rules are not hard-wired into the rewriting engine: they are written in a C-like language and are automatically processed and incorporated into the rewriting engine. That makes it possible for end-users to add their own rules or to provide sets of rules that are adapted to certain specific domains or purposes.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{A. Villanueva (Ed.): PROLE 2016\\
EPTCS 237, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.237.3}{10.4204/EPTCS.237.3}}

